Disagreement-Guided Weak-to-Strong Routing

Small language models are increasingly deployed on edge devices and robotic systems to meet cost and latency constraints, yet their limited capabilities can make reliable deployment challenging. Stronger models can provide assistance when needed, but deciding when to route a weak-model response to a stronger model often relies on signals of response correctness. In open-ended and agentic tasks, however, obtaining such signals can require costly ground-truth supervision that is difficult to obtain at scale. We revisit the foundations of weak-to-strong routing and ask whether routing decisions can instead be guided by signals that do not require ground-truth supervision. We first characterize the optimal weak-to-strong routing policy, while allowing for multiple weak-model responses generated through local inference. Building on this characterization, we derive a principled approximation to the optimal routing based on model-to-model comparison. In particular, we introduce a notion of model disagreement that can be measured directly from model-generated responses, without ground-truth supervision. Importantly, the approximation becomes increasingly accurate as the strong model becomes a better proxy for the ground-truth distribution. Across agentic and single-turn tasks, our approach effectively navigates the trade-off between routing cost and response accuracy without ground-truth supervision. Moreover, even when ground-truth correctness signals are available for training, disagreement-based routing can outperform methods trained directly to predict correctness

==> drafting.tex <==
\section{Finite-Sample Routing via Learned Probes}
\label{sec:experiments}

The population analysis of Section~\ref{subsec:population_comparison} established that corrected disagreement closely tracks the Bayes-optimal routing gain. At test time, however, the router cannot evaluate expectations under the strong model's distribution: it observes only the prompt $p$, generates candidate responses from the local weak model, and must autonomously decide whether to defer. 

To bridge this gap, we must estimate these population quantities from finite samples. The key advantage of our formulation is that it swaps the intractable problem of estimating ground-truth correctness for the highly tractable problem of estimating model disagreement. Because disagreement can be measured directly from model rollouts, we completely bypass the need for human annotations. We construct empirical disagreement targets using offline samples from both models, and train probes on the weak model's internal representations to predict them. By minimizing a proper scoring rule, these probes yield consistent estimators of the true disagreement probabilities. At inference, the weak model simply evaluates its own activations through the probes, allowing it to make autonomous routing decisions without any ground-truth labels or test-time queries to the strong model.

\subsection{The Learning Framework}
\label{subsec:finite_learning}

To estimate the components of the corrected-disagreement score, we frame the task as a general supervised learning problem. For a given input feature representation $\boldsymbol{\phi}(\cdot)$ and a target empirical probability $t \in [0, 1]$, we seek a probe function $f$ that minimizes a proper scoring rule over a training dataset $\mathcal{S} = \{(\boldsymbol{\phi}_i, t_i)\}$. 

\paragraph{Optimization and loss.}
We parameterize each probe $f$ as a linear map followed by a sigmoid activation: $f(x) = \sigma(w^\top x + b)$. We learn the parameters $(w, b)$ by minimizing the soft-label binary cross-entropy (BCE) loss with $\ell_2$ regularization:
\begin{equation}
\label{eq:bce_loss}
\mathcal{L}(w, b) = -\frac{1}{|\mathcal{S}|} \sum_{(\boldsymbol{\phi}, t) \in \mathcal{S}} \Big[ t \log f(\boldsymbol{\phi}) + (1 - t) \log \big(1 - f(\boldsymbol{\phi})\big) \Big] + \frac{\lambda}{2} \|w\|_2^2.
\end{equation}
Because BCE is a strictly proper scoring rule, the global minimizer guarantees $f^*(\boldsymbol{\phi}) = \mathbb{E}[t \mid \boldsymbol{\phi}]$. Thus, training on unbiased Monte Carlo targets $t$ yields a consistent estimator of the underlying population probability. 

\paragraph{Representations $\boldsymbol{\phi}(\cdot)$.}
Because the weak model is executed locally, its internal hidden activations provide a rich, zero-cost feature space. We extract two types of representations:
\begin{itemize}
    \item $\boldsymbol{\phi}(p) \in \mathbb{R}^d$: A representation of the prompt alone, extracted as the hidden state at the final prompt token. 
    \item $\boldsymbol{\phi}(p, y_w) \in \mathbb{R}^d$: A joint representation of the prompt and a candidate weak response, extracted as the mean hidden state across the generated response tokens.
\end{itemize}
In our experiments, these features are extracted from a single middle layer of the weak model ($\ell = 16$ of $28$ for the 1.5B--1.7B models; ablations over layers and pooling strategies are deferred to Appendix~\ref{app:probes}).

\paragraph{Empirical targets $t$.}
To generate the supervision targets, we collect a dataset of offline rollouts $\mathcal{D}_{\text{train}} = \{p_j\}_{j=1}^M$. For each prompt, we sample $K$ completions from both the weak and strong models. We evaluate agreement between any two completions using an indicator $A(y, y') \in \{0, 1\}$. In practice, $A(y, y')$ is evaluated via deterministic parsing, programmatic execution, or by simply prompting the teacher model to judge whether a candidate aligns with its own answer. This agreement check is highly scalable, requires no ground truth, and is used strictly offline to construct the targets.

We train two distinct probes using this data. The \textbf{weak--strong disagreement probe} ($\widehat{f}_d$) evaluates candidate-specific divergence; it takes the joint features $\boldsymbol{\phi}(p, y_w)$ as input and is trained to predict the empirical disagreement target:
\begin{equation}
\label{eq:target_d}
\widehat{d}(p, y_w) := 1 - \frac{1}{K} \sum_{k=1}^K A(y_w, y_{s,k}).
\end{equation}
The \textbf{self-disagreement probe} ($\widehat{f}_g$) evaluates the intrinsic difficulty of the prompt, independent of any specific weak response. It takes the prompt-only features $\boldsymbol{\phi}(p)$ as input and is trained to predict the empirical inconsistency among independent strong rollouts:
\begin{equation}
\label{eq:target_g}
\widehat{g}(p) := 1 - \frac{1}{K(K-1)} \sum_{k=1}^K \sum_{k' \neq k} A(y_{s,k}, y_{s,k'}).
\end{equation}

\paragraph{Test-time routing score.}
At inference, the weak model generates a candidate $y_w$, extracts the zero-cost representations $\boldsymbol{\phi}(p)$ and $\boldsymbol{\phi}(p, y_w)$, and passes them through the learned probes. The final corrected-disagreement score is seamlessly assembled as:
\begin{equation}
\label{eq:learned_score}
\widehat{S}_{\mathrm{cd}}(p, y_w) := \widehat{f}_d\big(\boldsymbol{\phi}(p, y_w)\big) - \widehat{f}_g\big(\boldsymbol{\phi}(p)\big).
\end{equation}
The routing threshold $\tau$ is calibrated via out-of-fold predictions on $\mathcal{D}_{\text{train}}$ to satisfy a target query budget $B_s$. 

\paragraph{Candidate selection.}
When the weak model generates multiple candidate responses ($N > 1$), a selection policy must choose which output to return if the cascade decides not to route. While one could naturally select the candidate with the lowest predicted disagreement $\widehat{f}_d(\boldsymbol{\phi}(p, y_w))$, many other rules are admissible, such as plurality voting or likelihood ranking. Because our primary focus is evaluating the efficacy of the \emph{routing} signal, we fix the selection rule (e.g., plurality vote) identically across all evaluated baselines in our multi-sample experiments. This ensures a fair comparison where the performance differences stem entirely from the routing mechanism. A comprehensive ablation studying alternative selection policies is provided in Appendix~\ref{app:selection}.

\subsection{Agentic Environments: Routing Without Ground Truth}
\label{subsec:finite_agentic}

We begin our empirical evaluation in interactive, multi-step agentic environments. This is the regime our method is most explicitly designed for, as step-level correctness is fundamentally ill-defined. In long-horizon tasks, an action's utility is realized only through delayed environmental feedback many steps later. Furthermore, evaluating intermediate steps using external LLM judges is notoriously noisy and struggles with credit assignment. 

In contrast, step-level \emph{disagreement} is objective and well-defined: two candidate actions are the same if they call the same tool with the same arguments, or induce the same environment transition. Disagreement can therefore be collected effortlessly without human labels, task-reward engineering, or fragile LLM judges.

\paragraph{Setting and baselines ($N=1$).}
Because an agent must sequentially propose and execute actions, we evaluate this setting in the one-shot regime ($N=1$): the weak model produces a single candidate action at each step, and the router decides whether to defer to the strong model. In this regime, consistency-based signals (like self-consistency and semantic entropy) are mathematically undefined, as a single sample constitutes its own trivial cluster. Correctness-supervised probes are similarly unavailable. We therefore compare our learned scores ($\widehat{f}_d$ and $\widehat{S}_{\mathrm{cd}}$) against the strongest available label-free baselines: token-level predictive uncertainty (mean token entropy) and random routing.

\paragraph{Environments and on-policy data collection.}
We evaluate on two environments: \textbf{BFCL multi-turn} (stateful function-calling across simulated backends; Qwen3-8B routed to GPT-5-mini) and \textbf{WebShop} (interactive e-commerce search and navigation; Qwen3-8B routed to a task-specialized RL policy). 

To prevent distribution shift during training, we gather interactions iteratively using a DAgger-style schedule: Phase~1 rolls out the autonomous weak policy, recording state histories and sampled actions to train the initial probes. Phase~$m \ge 2$ rolls out the cascading agent using the current probes, querying the strong model when $\widehat{S}_{\mathrm{cd}} > \tau$. Visited states are labeled for disagreement and aggregated to refine the probes. Final performance is measured by end-to-end task completion rates on held-out environments.

\TODO{Table: BFCL and WebShop task success at realized action budgets of 20/30/50\%, five runs per configuration on the held-out tasks, task-bootstrap standard errors.}

\subsection{Controlled Ablations on Single-Turn Benchmarks}
\label{subsec:finite_single_turn}

To rigorously study the properties of our routing signals against established baselines, we evaluate them on single-turn reasoning tasks. Because these benchmarks possess canonical gold answers, we can run controlled ablations that are impossible in the agentic setting: we can measure performance against a proxy-reward trained directly on ground truth, and we can vary the sample budget $N$ to compare against consistency-based methods. 

\paragraph{Benchmarks and model pairs.}
We use three diverse datasets: \textbf{\textsc{Math}-500} (Qwen2.5-1.5B-Instruct $\to$ GPT-4o-mini; offline equivalence $A$ is exact math match), \textbf{\textsc{Spider}} (Qwen3-1.7B $\to$ OmniSQL-7B; $A$ is identical SQL execution), and \textbf{\textsc{AceCode}} (Qwen2.5-Coder-1.5B-Instruct $\to$ Qwen3-Coder-30B-A3B-Instruct; $A$ is identical behavior on hidden unit tests).

\paragraph{One-shot routing ($N=1$).}
In the single-sample setting, we compare our probes against token-level uncertainty and a \textbf{proxy correctness} baseline ($\widehat{f}_c$). The correctness baseline is trained on the exact same features $\boldsymbol{\phi}(p, y_w)$ but supervised directly by the gold indicator $A(y_w, Y)$. We stress that this baseline operates with an unfair informational advantage, serving as an oracle reference representing methods with access to ground truth rather than a peer running under the same label-free constraints.

\paragraph{Uniform sampling ($N=n$).}
We also evaluate cascades where each prompt receives $n$ weak samples ($n \in \{4, 8, 16\}$). This allows us to benchmark against multi-sample approaches: \textbf{Self-Consistency} (plurality vote share) and \textbf{Semantic Entropy}. Both baselines require an automated mechanism to decide whether two free-form responses belong to the same answer cluster at test time. While trivial on closed-form math benchmarks, grouping open-ended code or SQL outputs requires expensive test-time LLM judges or bidirectional NLI entailment. We evaluate these practical clustering approximations, alongside an unrealistic offline-oracle ceiling (execution sandboxes). 

We emphasize the inherent asymmetry in test-time compute here: consistency-based routing signals require generating $n$ completions \emph{and} running $O(n^2)$ semantic similarity checks at inference, whereas our learned probes require only a single forward pass over the selected candidate's internal representations. 

\TODO{Tables: for each benchmark, accuracy at realized budgets 5/10/15/30\% for $N=1$ and for $N\in\{4,8,16\}$.}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

